Learning in games with continuous action sets and unknown payoff functions

This paper examines the convergence of no-regret learning in games with continuous action sets. For concreteness, we focus on learning via "dual averaging", a widely used class of no-regret learning schemes where players take small steps along their individual payoff gradients and then "mirror" the output back to their action sets. In terms of feedback, we assume that players can only estimate their payoff gradients up to a zero-mean error with bounded variance. To study the convergence of the induced sequence of play, we introduce the notion of variational stability, and we show that stable equilibria are locally attracting with high probability whereas globally stable equilibria are globally attracting with probability 1. We also discuss some applications to mixed-strategy learning in finite games, and we provide explicit estimates of the method's convergence speed.

==> Figures/Stability.tex <==
%----------------------------------------------------------------------
%%% MD
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\colorlet{BackgroundColor}{DodgerBlue!40!MidnightBlue}

\footnotesize
\begin{tikzpicture}
[scale=1,
>=stealth,
vecstyle/.style = {->, line width=.5pt},
edgestyle/.style={-, line width=.5pt},
%nodestyle/.style={circle, fill=Black,inner sep = .5pt},
nodestyle/.style = {circle,fill=black,inner sep=0, minimum size=2},
plotstyle/.style={color=DarkGreen!80!Cyan,thick}]

\def\radius{2.5}
\def\costhirty{0.8660256}
\def\cosfortyfive{0.7071068}
\def\veclength{.5}

\coordinate (Nash-coord) at (3,0);
\coordinate (stable-coord) at (0,0);
\coordinate (monotone-coord) at (-3.5,0);
\coordinate (potential-coord) at (-7,0);

%\coordinate (static) at (0,0);
%\coordinate (stochastic) at (-2,0);
%\coordinate (games) at (2,0);
%
%\filldraw [fill = DodgerBlue!10!white, rounded corners = 5] (-6,-3.5) rectangle (6,2);
%
%\def\static{(static) ellipse [x radius = 1.5, y radius = 1]}
%\def\stochastic{(stochastic) ellipse [x radius = 3.75, y radius = 1.75]}
%\def\games{(games) ellipse [x radius = 3.75, y radius = 1.75]}
%
%\fill [DarkGreen!50] \static;
%\fill [DodgerBlue!80, fill opacity = .4] \stochastic;
%\fill [DarkGreen!40, fill opacity = .4] \games;
%
%\draw \static;
%\draw \stochastic;
%\draw \games;

\node (Nash) [draw=black, align=center, fill = DodgerBlue!10!white, rounded corners = 5]
at (Nash-coord)
{%
\textsf{\bfseries Nash equilibrium}
\\[.5ex]
$\braket{\payv(\eq)}{x - \eq} \leq 0$};

\node (stable) [draw=black, align=center, fill = DodgerBlue!10!white, rounded corners = 5]
at (stable-coord)
{%
\textsf{\bfseries Variatonal stability}
\\[.5ex]
$\braket{\payv(x)}{x - \eq} \leq 0$};

\node (stable-Hess) at (stable.south) [below] {$\hessmat(\eq) \ml 0$};

\node (monotone) [draw=black, align=center, fill = DodgerBlue!10!white, rounded corners = 5]
at (monotone-coord)
{%
\textsf{\bfseries Monotone games}
\\[.5ex]
$\braket{\payv(x') - \payv(x)}{x' - x} \leq 0$};

\node (monotone-Hess) at (monotone.south) [below] {$\hessmat(x) \ml 0$};

\node (potential) [draw=black, align=center, fill = DodgerBlue!10!white, rounded corners = 5]
at (potential-coord)
{%
\textsf{\bfseries Concave potential}
\\[.5ex]
$\payv(x) = \nabla\pot(x)$};

\node (potential-Hess) at (potential.south) [below] {$\nabla^{2}\pot(x) \ml 0$};

\draw [-implies,double equal sign distance] (potential) to (monotone);
\draw [-implies,double equal sign distance] (monotone) to (stable);
\draw [-implies,double equal sign distance] (stable) to (Nash);

\end{tikzpicture}
